Local Galois Symbols on E x E

This article is the first part of a two-part work on the Albanese kernel T_F(E x E), for an elliptic curve E over F. The main result furnishes information, for any odd prime p, about the kernel and image of the Galois symbol map from T_F(E \times E)/p to the Galois cohomology group H^2(F, E[p] (x) E[p]), for F a p-adic field and E/F ordinary, without requiring that the p-torsion points are F-rational. A key step is to show that the image is zero when the Galois module E[p] is non-semisimple. The forthcoming second part will deal with global questions.

==> biblio.tex <==
%X-Sun-Data-Type: default
%X-Sun-Data-Name: biblio.tex
%X-Sun-Charset: us-ascii
%X-Sun-Content-Lines: 47

\addcontentsline{toc}{section}{Bibliography}
\begin{thebibliography}{99}

\bibitem[BT]{BT} H.~Bass and J.~Tate, The Milnor ring of a global field,
in {\it Algebraic $K$-theory, II: "Classical" algebraic $K$-theory
and connections with arithmetic}, 349--446, Lecture Notes in Math.
{\bf 342}, Springer-Verlag (1973).

\bibitem[Bl]{Bl}
S. Bloch, {\it Lectures on Algebraic Cycles}, Duke University
Press (1980).

\bibitem[Br]{Brown} K.~Brown, {\it Cohomology of groups},
Lecture Notes in Math., Springer-Verlag.

\bibitem[CT]{CT} J.-L.~Colliot-Th\'el\`ne, Cycles alg\'ebriques de
torsion et $K$-th\'eorie alg\'ebrique, in {\it Arithmetic
Algebraic Geometry}, Trento, Lecture Notes in Math. {\bf 1553}
(1991), Springer-Verlag.

\bibitem[F]{F} W.~Fulton, {\it Intersection theory} (second
edition), Springer-Verlag (1998).

\bibitem[J]{J} U.~Jannsen, {\it Continuous étale cohomology},
Math. Annalen  {\bf 280}  (1988), no. 2, 207--245.

\bibitem[Ka]{Kahn} B.~Kahn, 

\bibitem[L1]{Lang1} S.~Lang, Algebraic groups over finite fields.
Amer. J. Math. {\bf 78} (1956), 555--563. (1956), 555--563.

\bibitem[L2]{Lang2} S.~Lang, {\it Algebraic Number Theory},
Addison-Wesley (1970).

\bibitem[Mac]{Mac} W.~McCallum, 

\bibitem[{[Maz]}]{Mazur} B.~Mazur, 

\bibitem[Mi1]{Mi1} J.S.~Milne, {\it Etale cohomology}, Princeton
University Press (1980), Princeton, NJ.

\bibitem[Mi2]{Mi2} J.S.~Milne, {\it Arithmetic duality theorems},
Perspectives in Math. {\bf 1}, Academic Press (1986).

\bibitem[M]{M} J.~Milnor, {\it Algebraic $K$-theory}, Annals of
Math. Studies {\bf 72}, Princeton University Press (1971).

\bibitem[ParS]{ParS} R.~Parimala and V.~Suresh, Zero cycles on
quadric fibrations: Finiteness theorems and the cycle map,
Inventiones Math. {\bf 122} (1995), 83--117.

\bibitem[R]{R} W.~Raskind, Higher $l$-adic Abel-Jacobi mappings
and filtrations on Chow groups.  Duke Math. Journal  {\bf 78}
(1995), no. 1, 33--57.

\bibitem[R-S]{RS} W.~Raskind and M.~Spiess,  Milnor $K$-groups and zero-cycles on
products of curves over $p$-adic fields, Compositio Math. {\bf
121} (2000), no. 1, 1--33.

\bibitem[Ray1]{Raynaud} M.~Raynaud, Sc\'emas en groupes de type
$(p,\dots,p)$, Bull. Soc. Math. France {\bf 102}, (1974),
241--280.

\bibitem[Ray2]{Raynaud2} M.~Raynaud, in {\it Local fields}, Driebergen, 78--85.

\bibitem[SGA4]{SGA} A.~Grothendieck, S\'eminaire de G\'eometrie Alg\'ebrique $4$

\bibitem[Se1]{Serre1} J.-P.~Serre, Propri\'et\'es galoisiennes des points
d'ordre fini des courbes elliptiques, Inventiones Math. {\bf 15}
(1972), 259--331.

\bibitem[Se2]{Serre2} J.-P.~Serre, {\it Abelian $\ell$-adic representations and
elliptic curves} (second edition), Addison-Wesley (1989).

\bibitem[Se3]{Serre3} J.-P.~Serre, {\it Local fields}, English translation of
{\it Corps Locaux}, Graduate Texts in Mathematics {\bf 67},
Springer-Verlag (1979).

\bibitem[Se4]{Serre4} J.-P.~Serre, 

\bibitem[Sil1]{Silv1} {\it The arithmetic of elliptic curves},
Graduate Texts in Math. {\bf 106}, Springer-Verlag (1986)

\bibitem[Sil2]{Silv2} {\it Advanced topics in the arithmetic of
elliptic curves} (corrected second printing), Graduate Texts in
Math. {\bf 151}, Springer-Verlag (1999).

\bibitem[So]{So} M.~Somekawa,  On Milnor $K$-groups attached to semi-abelian
varieties, $K$-Theory {\bf 4} (1990), no. 2, 105--119.

\bibitem[Spa]{Spanier} E.H.~Spanier, {\it Algebraic Topology},
McGraw-Hill (1966).

\bibitem[Sp]{Sp} M.~Spiess, 

\bibitem[Ta1]{Tate1}, J.~Tate, Duality theorems in Galois cohomology
over number fields. 1963  Proceedings of the International
Congress of Mathematicians, Stockholm (1962), 288--295.

\bibitem[Ta2]{Tate2}, J.~Tate,  $p$-divisible groups,
Proceedings of the Conference on {\it Local Fields}, Driebergen,
158--183, Springer-Verlag (1967).

\bibitem[Ta3]{Tate3} J.~Tate, $K_2$ and Galois cohomology, Inventiones
Math. {\bf 36} (1976), 257--274.

\bibitem[Ta4]{Tate4} J.~Tate, in {\it Modular forms and Fermat's last
theorem}, ed. by G.~Cornell, J.~Silverman and G.~Stevens (2000).

\bibitem[W]{W} A.~Weil, {\it Foundations of algebraic geometry} (second edition),
American Mathematical Society, Providence, R.I. (1962)


\end{thebibliography}

\vskip 0.2in

\noindent{Dinakar Ramakrishnan}, \emph{California Institute of
Technology, Pasadena, CA 91125, USA}

\medskip

\noindent{Jacob Murre}, \emph{University of Leiden, Leiden,
Netherlands}


